Online Discovery of Evolving Groups over Massive-Scale Trajectory Streams

The increasing pervasiveness of object tracking technologies leads to huge volumes of spatiotemporal data collected in the form of trajectory streams. The discovery of useful group patterns from moving objects' movement behaviours in trajectory streams is critical for real-time applications ranging from transportation management to military surveillance. Motivated by this, we first propose a novel pattern, called evolving group, which models the unusual group events of moving objects that travel together within density connected clusters in evolving streaming trajectories. Our theoretical analysis and empirical study on the Osaka Pedestrian data and Beijing Taxi data demonstrate its effectiveness in capturing the development, evolution, and trend of group events of moving objects in streaming context. Moreover, we propose a discovery method that efficiently supports online detection of evolving groups over massive-scale trajectory streams using a sliding window. It contains three phases along with a set of novel optimization techniques designed to minimize the computation costs. Furthermore, to scale to huge workloads over evolving streams, we extend our discovery method to a parallel framework by using a sector-based partition. Our comprehensive empirical study demonstrates that our online discovery framework is effective and efficient on real-world high-volume trajectory streams.

==> 8authorbio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
% \vspace{-8mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/lan}}]{Ruoshan Lan}
received her B.S. degree in Computer Science from the School of Computer and Control Engineering of Yantai University, China in 2017. 
She is currently working toward the M.S. degree in Software Systems Engineering at the Department of Computer Science of RWTH Aachen University, Germany. Her research interests include data mining, machine learning and artificial intelligent.
\end{IEEEbiography}

% \vspace{-8mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/yu}}]{Yanwei Yu}
(S'12-M'16) received his Ph.D. degree in Computer Science from University of Science and Technology Beijing, China in 2014. From 2012 to 2013, he was a visiting scholar in the Worcester Polytechnic Institute, Massachusetts. From 2016 to 2018, he was a postdoctoral associate at the College of Information Sciences and Technology, Pennsylvania State University.
He is currently an associate professor at the Department of Computer Science and Technology, Ocean University of China. His research interests include data mining, machine learning and distributed computing. He is a member of IEEE. Corresponding author of this paper.
\end{IEEEbiography}

% \vspace{-8mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/cao}}]{Lei Cao}
(M'14) received his Ph.D. degree in Computer Science from Worcester Polytechnic Institute, USA in 2016. From 2015 to 2016, he worked as researcher at Thomas J. Watson Research Center, IBM.
He is currently a postdoctoral associate at the Computer Science and Artificial Intelligence Laboratory, Massachusetts Institute of Technology. His research interests include data mining and machine learning. He is a member of the IEEE.
\end{IEEEbiography}

% \vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/song}}]{Peng Song}
(M'16) received the B.S. degree from Shandong University of Science and Technology, China, in 2006. He received the M.S. and Ph.D. degrees from Southeast University, China, in 2009 and 2014, respectively. From 2009 to 2011, he worked as a software engineer at Motorola. He is currently an associate professor with the School of Computer and Control Engineering of Yantai University. His research interests include affective computing, speech signal processing and machine learning. He is a member of the IEEE.
\end{IEEEbiography}

% \vspace{-10mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/wang}}]{Yingjie Wang}
(M'16) received the Ph.D. degree from the School of Computer Science and Technology of Harbin Engineering University, China, in 2015. From 2013 to 2014, she was a visiting scholar in the Georgia State University, Atlanta, Georgia. She is currently an associate professor with the School of Computer and Control Engineering of Yantai University. Her research interests include crowd-sourcing networks, trusted computing and artificial intelligent. She is a member of the IEEE.
\end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage
\balance

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

% \vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
